TReCiM: Lower Power and Temperature-Resilient Multibit 2FeFET-1T Compute-in-Memory Design

Compute-in-memory (CiM) emerges as a promising solution to solve hardware challenges in artificial intelligence (AI) and the Internet of Things (IoT), particularly addressing the "memory wall" issue. By utilizing nonvolatile memory (NVM) devices in a crossbar structure, CiM efficiently accelerates multiply-accumulate (MAC) computations, the crucial operations in neural networks and other AI models. Among various NVM devices, Ferroelectric FET (FeFET) is particularly appealing for ultra-low-power CiM arrays due to its CMOS compatibility, voltage-driven write/read mechanisms and high ION/IOFF ratio. Moreover, subthreshold-operated FeFETs, which operate at scaling voltages in the subthreshold region, can further minimize the power consumption of CiM array. However, subthreshold-FeFETs are susceptible to temperature drift, resulting in computation accuracy degradation. Existing solutions exhibit weak temperature resilience at larger array size and only support 1-bit. In this paper, we propose TReCiM, an ultra-low-power temperature-resilient multibit 2FeFET-1T CiM design that reliably performs MAC operations in the subthreshold-FeFET region with temperature ranging from 0 to 85 degrees Celcius at scale. We benchmark our design using NeuroSim framework in the context of VGG-8 neural network architecture running the CIFAR-10 dataset. Benchmarking results suggest that when considering temperature drift impact, our proposed TReCiM array achieves 91.31% accuracy, with 1.86% accuracy improvement compared to existing 1-bit 2T-1FeFET CiM array. Furthermore, our proposed design achieves 48.03 TOPS/W energy efficiency at system level, comparable to existing designs with smaller technology feature sizes.

==> tabs/compare.tex <==
\begin{table*}[]
\centering
\caption{Comparisons of   CAM Designs}
%\vspace{-3mm}
\label{tab:comparison}
\resizebox{2\columnwidth}{!}{
\begin{tabular}{|c|ccccccc|}
\bottomrule
\textbf{Designs} & \textbf{Device}& \textbf{Cell Structure}\eat{&\textbf{Matching scheme}}& \textbf{Type}&\textbf{Search energy per bit $(fJ)$} & \textbf{Latency $(ps)$}& \textbf{Area per bit ($\mu m^2$)}& \textbf{NVM/MOS node $(nm)$}   \\\toprule\bottomrule
\textbf{16T CMOS}~\cite{pagiamtzis2006content}&CMOS&16T&BCAM&0.59 (\textcolor{red}{$\times9.8$})&582.4 (\textcolor{red}{$\times1.6$})&1.12 ($\times9.3$)&-/45\\
\textbf{DAC'22}~\cite{cai2022energy}&FeFET&2T-1FeFET&BCAM&0.116 (\textcolor{red}{$\times1.9$})&401.4 (\textcolor{red}{$\times1.1$})&0.36 ($\times3$)&45/45
\\
\textbf{Nat Ele'19}~\cite{ni2019ferroelectric}&FeFET&2FeFET&TCAM&0.40 (\textcolor{red}{$\times6.7$})&360 (\textcolor{red}{$\times1$})&0.15 ($\times1.2$)&45/-
\\
\textbf{DATE'21 (P$^\#$)}~\cite{qian2021energy}&FeFET&2FeFET-1T\eat{&Exact}&TCAM&0.195 (\textcolor{red}{$\times3.3$})&252.8 (\textcolor{red}{$\times0.7$})&0.36 ($\times3$)& 45/45
\\
\textbf{DATE'21 (PF$^\#$)}~\cite{qian2021energy}&FeFET&2FeFET-2T\eat{&Exact}&TCAM&0.073 (\textcolor{red}{$\times1.2$})&1430 (\textcolor{red}{$\times3.8$})&0.44 ($\times3.6$)& 45/45
\\
\textbf{JSSC'13}~\cite{li20131}&PCM&2T-2R\eat{&Exact}&TCAM&0.55 (\textcolor{red}{$\times9.2$})&350.6 (\textcolor{red}{$\times0.9$})&0.41 ($\times3.4$)&90/90
\\
% \textbf{JSSC'17}~\cite{chang20173t1r}&ReRAM&3T-1R\eat{&Exact}&TCAM&-$^\star$&-$^\star$&-$^\star$&90/90\\
\textbf{NC'20}~\cite{li2020analog}&ReRAM&6T-2R\eat{&Threshold}&ACAM&0.52 (\textcolor{red}{$\times8.7$})&110 (\textcolor{red}{$\times0.3$})&0.51$^\P$ ($\times4.2$)&50/180
\\
\textbf{TED'20}~\cite{yin2020fecam}&FeFET&2FeFET\eat{&Exact/Threshold}&MCAM/ACAM&0.182/0.069 (\textcolor{red}{$\times3$/$\times1.2$})&-&0.05($\times0.4$)&45/45
\\
% \textbf{SR'21$^*$}~\cite{kazemi2022achieving}&FeFET&2FeFET\eat{&Exact}&MCAM&-$^\star$&-$^\star$&-$^\star$&28/-\\
\textbf{IEDM'20}~\cite{li2020scalable}&FeFET&2FeFET-1T$^\ddagger$\eat{&Exact}&MCAM&0.292 (\textcolor{red}{$\times4.9$})&422 (\textcolor{red}{$\times1.1$})&0.03$^\&$ ($\times0.2$)& 28/-
\\
\textbf{This work (P)}&FeFET&2FeFET-1T&MCAM&0.06$^\dagger$ ($\times1$)&371.8 ($\times1$)&0.12 ($\times1$)& 45/40
\\
 \textbf{This work (PF)}&FeFET&2FeFET-2T\eat{&Exact}&MCAM& 0.039$^\dagger$&2040 &0.146& 45/40
 \\
\toprule
\end{tabular}
}
\flushleft
$\dagger$: Results are evaluated under 32 cells per word. 
$\ddagger$: Two ML branches for one stored vector. \eat{$*$: CAM with novel distance functions. $\star$: Single-cell metrics are not reported.} $\#$: Precharge and precharge-free. 
$\P$: Reported based on 16nm design rules.
%$*$: Results is based on 32 cells per word.
$\&$: Smaller cell size due to 28nm technology node. 


\end{table*}



==> tabs/datasets.tex <==
\begin{table}[]
% \vspace{-3mm}
\centering
\caption{Datasets ($n$: feature size, $K$: number of classes)}
% \vspace{-3mm}
\label{tab:benchmark}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{|c|ccccc|}
\toprule
\textbf{Dataset}& $n$ & $K$ & \shortstack{\textbf{Train}\\ \textbf{Size}} & \shortstack{\textbf{Test}\\ \textbf{Size}} & \textbf{Description}             \\ \midrule
\textbf{ISOLET} & 617               & 26         & 6,238               & 1,559              & Voice Recognition~\cite{Isolet}              \\
\textbf{UCIHAR} & 561               & 12          & 6,213                & 1,554               & Physical Activity Monitoring~\cite{anguita2012human} \\ 
% \textbf{FACE}   & 608               & 2         & 522,441             & 2,494              & Face Recognition\cite{angelova2005pruning}\\ 
% \textbf{PECAN} & 312             & 3          & 22,290  &  5,574       & Urban Electricity Prediction~\cite{pecan} \\ 
% \textbf{MNIST} & 784             & 10        &  60,000   & 10,000       & Handwritten Recongition~\cite{lecun1998gradient}\\ 
\textbf{PAMAP} &  75             &  5        &  611,142  & 101,582           & Human Activity Recognition~\cite{reiss2012introducing}           \\
\bottomrule
\end{tabular}
}
% \vspace{-1ex}
\end{table}

==> tabs/operations.tex <==

\begin{table}[]
% \vspace{-3mm}
\centering
\caption{Operation summary of a 3-bit SEE-MCAM.}
% \vspace{-3mm}
\label{tab:operation}
\resizebox{1\columnwidth}{!}{
\begin{tabular}{|c|cccccccc|}
\toprule
% \multirow{1}{*}{\textbf{Mode}} & \eat{\textbf{$\text{WL}_\text{1}$/$\text{WL}_\text{2}$}  &}\textbf{S/$\bar{\text{S}}$} & \textbf{$\text{SL}_\text{1}$/$\text{SL}_\text{2}$ $(V)$} & \textbf{D $(V)$} & \textbf{ML} \\ \midrule
% \textbf{Write `00'} & $-4 V (65 ns)$/$-4V (180ns)$  & 00/11       & \multirow{4}{*}{0/0}&-&-\\ 
% \textbf{Write `01'} & $-4 V (86 ns)$/$-4V (118ns)$  & 01/10       & &-&-\\ 
% \textbf{Write `10'} & $-4 V (118 ns)$/$-4V (86ns)$  & 10/01       & &-&-\\
% \textbf{Write `11'} & $-4 V (180 ns)$/$-4V (65 ns)$  & 11/00      & &-&-\\ \midrule
\shortstack{\textbf{$D$}\\\textbf{ML}}& \shortstack{\textbf{Stored}\\ \textbf{`000'}} & \shortstack{\textbf{Stored}\\ \textbf{`001'}}  & \shortstack{\textbf{Stored}\\ \textbf{`010'}}  & \shortstack{\textbf{Stored}\\ \textbf{`011'}} & \shortstack{\textbf{Stored}\\ \textbf{`100'}}  & \shortstack{\textbf{Stored}\\ \textbf{`101'}}  & \shortstack{\textbf{Stored}\\ \textbf{`110'}}  & \shortstack{\textbf{Stored}\\ \textbf{`111'}}  \\
\midrule
\shortstack{\textbf{Search}\\\textbf{`000'}}&  \makecell{\textit{L}\\\textit{M}} &  \makecell{H\\MM} &  \makecell{H\\MM} & \makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`001'}}&  \makecell{H\\MM} &  \makecell{\textit{L}\\\textit{M}} &  \makecell{ H\\ MM} & \makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`010'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{ \textit{L}\\ \textit{M}} & \makecell{ H\\ MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`011'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{ H\\ MM} & \makecell{ \textit{L}\\ \textit{M}}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`100'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{H\\MM} & \makecell{ H\\ MM}&\makecell{\textit{L}\\\textit{M}}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`101'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{H\\MM} & \makecell{H\\MM}&\makecell{H\\MM}&\makecell{\textit{L}\\\textit{M}}&\makecell{H\\MM}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`110'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{H\\MM} & \makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{\textit{L}\\\textit{M}}&\makecell{H\\MM} \\ \midrule
\shortstack{\textbf{Search}\\\textbf{`111'}}&  \makecell{H\\MM} &  \makecell{H\\MM} &  \makecell{H\\MM} & \makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{H\\MM}&\makecell{\textit{L}\\\textit{M}} \\ \midrule

\end{tabular}
}
\flushleft
For a given stored and input value pair. H/L indicates the high/low voltage level of the node $D$. M/MM indicates a match or mismatch state of ML.
% \vspace{-1ex}
\end{table}
